Two Birds and One Stone: Gaussian Interference Channel with a Shared Out-of-Band Relay of Limited Rate

The two-user Gaussian interference channel with a shared out-of-band relay is considered. The relay observes a linear combination of the source signals and broadcasts a common message to the two destinations, through a perfect link of fixed limited rate $R_0$ bits per channel use. The out-of-band nature of the relay is reflected by the fact that the common relay message does not interfere with the received signal at the two destinations. A general achievable rate is established, along with upper bounds on the capacity region for the Gaussian case. For $R_0$ values below a certain threshold, which depends on channel parameters, the capacity region of this channel is determined in this paper to within a constant gap of $\Delta=1.95$ bits. We identify interference regimes where a two-for-one gain in achievable rates is possible for every bit relayed, up to a constant approximation error. Instrumental to these results is a carefully-designed quantize-and-forward type of relay strategy along with a joint decoding scheme employed at destination ends. Further, we also study successive decoding strategies with optimal decoding order (corresponding to the order at which common, private, and relay messages are decoded), and show that successive decoding also achieves two-for-one gains asymptotically in regimes where a two-for-one gain is achievable by joint decoding; yet, successive decoding produces unbounded loss asymptotically when compared to joint decoding, in general.

==> ghf_vs_cf_tex.tex <==
%% Creator: Inkscape inkscape 0.48pre0, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'ghf_vs_cf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def{\svgwidth}{<desired width>}
%%   \input{<filename>.tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}

\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}
    \renewcommand\color[2][]{}%
  }
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}
    \renewcommand\transparent[1]{}%
  }
  \providecommand\rotatebox[2]{#2}
  \ifx\svgwidth\undefined
    \setlength{\unitlength}{446.61313477pt}
  \else
    \setlength{\unitlength}{\svgwidth}
  \fi
  \global\let\svgwidth\undefined
  \makeatother
  \begin{picture}(1,1.26785549)%
    \put(0,0){\includegraphics[width=\unitlength]{ghf_vs_cf.pdf}}%
    \put(0.77102524,0.68232488){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$q_1$}}}%
    \put(0.77102524,0.57484931){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$q_2$}}}%
    \put(0.87670954,1.10894177){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{user one}}}%
    \put(0.87681709,0.1683214){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{user two}}}%
    \put(0.01869627,0.38855833){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{source}}}%
    \put(0.66202737,0.38339359){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{relay }}}%
    \put(0.91945455,0.64172624){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$R_0=1$}}}%
  \end{picture}%
\endgroup


==> unirelay-asnoise.tex <==
\section{Treating Interference as Noise 
\label{sec:gaussian_interference_relay}}
A simple strategy 













The real advantage of GHF lies in a relay-interference channel,
where a single relay simultaneously assists more than one
receivers. The CF strategy requires the auxiliary random variable 
$\hat{Y_r}$ to be decoded uniquely at the receiver at the first step.  
Because the two receivers
in the interference channel may have different side information for
Wyner-Ziv decoding, the optimal $\hat{Y_r}$ for different receivers are in
general different. In contrast, GHF provides the possibility of
quantizing the relay observation with a single $\hat{Y_r}$, which, although
not optimal for either receiver at any finite noise level, becomes
optimal for both receivers asymptotically as noises go down to zero
(i.e.\ as the channel becomes deterministic). 

Consider a Gaussian interference channel as shown in
Fig.~\ref{fig:gauss-inter}
 \begin{subequations}
    \label{eq:7}
    \begin{align}
      Y_1&=h_{11}X_1+h_{21} X_2+Z_1\label{eq:y1}\\
      Y_2&=h_{12}X_1+h_{22} X_2+Z_2,
    \end{align}
  \end{subequations}
where the relay observes
\begin{equation}
Y_r=g_1 X_1 + g_2 X_2 + Z_r
\label{eq:yr}
\end{equation}
and has a common broadcast digital relay link of rate $R_0$ to both $Y_1$
and $Y_2$, where the noises $Z_1$, $Z_2$, $Z_r$ are i.i.d.\ Gaussian
random variables with zero mean and variance $N$, and where the
powers of $X_1$ and $X_2$ are constrained to be less than $P_1$ and
$P_2$ respectively. 

To avoid the case where the relay observation degenerates into one of
$Y_1$ and $Y_2$, we further assume
\begin{equation}
\frac{g_1}{g_2} \neq \frac{h_{11}}{h_{21}}, \qquad
\frac{g_1}{g_2} \neq \frac{h_{12}}{h_{22}}.
\label{eq:nondeg}
\end{equation}

We compare the rate improvement due to the relay against the baseline
rates where independent Gaussian codebooks with $X_1 \sim
\mathcal{N}(0,P_1)$, $X_2 \sim \mathcal{N}(0,P_2)$ are used at the
transmitters and where interference is always treated as noise: 
\begin{subequations}
\begin{align}
R_1 &= I(X_1;Y_1) = 
	\frac{1}{2} \log\left(1+\frac{h_{11}^2P_1}{h_{21}^2P_2+N} \right) \\
R_2 &= I(X_2;Y_2) = 
	\frac{1}{2} \log\left(1+\frac{h_{11}^2P_1}{h_{21}^2P_2+N} \right)
\end{align}
\end{subequations}
The main result of this section is that when interference is treated as noise, using a common digital relay
link of rate $R_0$, GHF can provide $R_0$ bits of rate improvement to
both users at the same time asymptotically as $N \rightarrow 0$, while
$h_{ij}$, $g_i$ and $P_i$ are kept fixed.  This is in contrast to CF
or AF strategies which do not provide the maximal $R_0$ bits of rate 
improvement. The next section generalizes this result to more complex encoding strategies for the interference channel where common-private power splitting is used.

\subsection{Rate Improvement using GHF \label{sec:ghf:analyze}}
We evaluate the achievable rate using GHF by assuming a joint Gaussian
auxiliary variable $\hat{Y_r}=Y_r+\eta $ with $\eta \sim\N(0,q)$. By Theorem 
\ref{thm:ghf}, the following rates are achievable using GHF 
\begin{subequations}
\label{eq:ghf_rate}
\begin{align}
R_1 = I(X_1;Y_1) + R_0 - I(\hat{Y_r};Y_r|X_1,Y_1); \\
R_2 = I(X_2;Y_2) + R_0 - I(\hat{Y_r};Y_r|X_2,Y_2).
\end{align}
\end{subequations}
subject to the condition that $p(\hat{y}_r|y_r)$ must satisfy
\begin{subequations}
\label{eq:R0_constraint}
\begin{align}
R_0 \le I(\hat{Y_r};Y_r|Y_1); \\
R_0 \le I(\hat{Y_r};Y_r|Y_2).
\end{align}
\end{subequations}
First, we evaluate
\begin{eqnarray}
\lefteqn{ I(\hat{Y_r};Y_r|X_1,Y_1)} \NoN \\
&&  = h(\hat{Y_r}|X_1,Y_1) - h(\hat{Y_r}|Y_r) \NoN \\
&& = \frac{1}{2} \log \left(2\pi e (\sigma^2_{\tilde{{Y_r}}} -
	\sigma_{\tilde{{Y_r}}\tilde{Y}_1}
	(\sigma_{\tilde{Y}_1}^2)^{-1} \sigma_{\tilde{Y}_1\tilde{{Y_r}}})
	\right) -
	\frac{1}{2} \log (2\pi e q) \NoN \\
&& = \frac{1}{2} \log \left( 1 + \frac{
	\left((g_2^2+h_{21}^2)P_2+N \right)N }
	{(h_{21}^2P_2+N) q} \right) 
\label{eq:rate_loss_1}
\end{eqnarray}
where $\tilde{{Y_r}}=g_2X_2+Z_r$ and $\tilde{Y}_1=h_{21}X_2+Z_1$.  Similarly,
\begin{equation}
I(\hat{Y_r};Y_r|X_2,Y_2) 
	= \frac{1}{2} \log \left( 1 + \frac{
	\left((g_1^2+h_{12}^2)P_1+N \right)N }
	{(h_{12}^2P_1+N) q} \right) 
\label{eq:rate_loss_2}
\end{equation}
We also need to evaluate
\begin{eqnarray}
\lefteqn{ I(\hat{Y_r};Y_r|Y_1) = h(\hat{Y_r}|Y_1) - h(\hat{Y_r}|Y_r)} \NoN \\
%\lefteqn{ I(\hat{Y_r};Y_r|Y_1)} \NoN \\
%&& = h(\hat{Y_r}|Y_1) - h(\hat{Y_r}|Y_r) \NoN \\
&& = \frac{1}{2} \log \left(2\pi e (\sigma^2_{\hat{Y_r}} - \sigma_{\hat{Y_r}Y_1}
	(\sigma_{Y_1}^2)^{-1} \sigma_{Y_1\hat{Y_r}}) \right) -
	\frac{1}{2} \log (2\pi e q) \NoN \\
%&& = \frac{1}{2} \log \left( 1 + \frac{g_1^2P_1+g_2^2P_2+N -
%	\frac{(g_1h_{11}P_1+g_2h_{21}P_2)^2}{h_{11}^2P_1+h_{21}^2P_2+N}} 
%	{q} \right) \NoN \\
&& = \frac{1}{2} \log \left( 1 + \frac{
	(g_1h_{21}-g_2h_{11})^2P_1P_2 + c_1 N}
	{(h_{11}^2P_1+h_{21}^2P_2+N) q} \right) 
\label{eq:Q_1}
\end{eqnarray}
where $c_1 = (g_1^2+h_{11}^2)P_1+(g_2^2+h_{21}^2)P_2+N$. 
Similarly,
\begin{equation}
I(\hat{Y_r};Y_r|Y_2) = \frac{1}{2} \log \left( 1 + \frac{
	(g_1h_{22}-g_2h_{12})^2P_1P_2 + c_2 N}
	{(h_{12}^2P_1+h_{22}^2P_2+N) q} \right)
\label{eq:Q_2}
\end{equation}
where $c_2 = (g_1^2+h_{12}^2)P_1+(g_2^2+h_{22}^2)P_2+N$. 


For any fixed $R_0$, we can always find $q$ that satisfies both
constraints in (\ref{eq:R0_constraint}).  In addition, as long as
(\ref{eq:nondeg}) is satisfied, we can find values for $q$ that
satisfy (\ref{eq:R0_constraint}) and do not go to zero as $N
\rightarrow 0$. In fact, the largest GHF rate is obtained by choosing
$q$ to satisfy the more stringent of (\ref{eq:R0_constraint}) with
equality. In this case, by (\ref{eq:Q_1}) and (\ref{eq:Q_2}), the
limiting value of $q$ as $N \rightarrow 0$ is
%\begin{multline}
%q = \frac{1}{2^{2R_0}-1} \min \left\{ 
%	\frac{(g_1h_{21}-g_2h_{11})^2P_1P_2}
%	{(h_{11}^2P_1+h_{21}^2P_2)} , \right.\\
%	\left.
%	\frac{(g_1h_{22}-g_2h_{12})^2P_1P_2} 
%	{(h_{12}^2P_1+h_{22}^2P_2)} \right\}
%\label{eq:ghf_asymptotic_q}
%\end{multline}
\begin{equation}
q = \frac{1}{2^{2R_0}-1} \min( a, b),
\label{eq:ghf_asymptotic_Q}
\end{equation}
where
\begin{subequations}
\begin{align}
a = \frac{(g_1h_{21}-g_2h_{11})^2P_1P_2} {(h_{11}^2P_1+h_{21}^2P_2)},\\
b = \frac{(g_1h_{22}-g_2h_{12})^2P_1P_2} {(h_{12}^2P_1+h_{22}^2P_2)}. 
\end{align}
\label{eq:definition_ab}
\end{subequations}
This value for $q$ is a constant bounded away from zero. 

Substituting this $q$ into (\ref{eq:rate_loss_1}) and
(\ref{eq:rate_loss_2}), we see that as $N \rightarrow 0$, both
$I(\hat{Y_r};Y_r|X_1,Y_1)$ and $I(\hat{Y_r};Y_r|X_2,Y_2)$ vanish, implying that
GHF achieves exactly $R_0$ bits in rate improvement for both users at
the same time.


\subsection{Rate Improvement using CF \label{sec:sim:cf}}
For a CF strategy to help both receivers in an interference channel at
the same time, we need a single $\hat{Y_r}$ that is uniquely decodable at both 
receivers. In this case, the achievable rate using CF is
\begin{subequations}
\label{eq:cf_rate}
\begin{align}
R_1 = I(X_1;Y_1,\hat{Y_r}) \\
R_2 = I(X_2;Y_2,\hat{Y_r}) 
\end{align}
\end{subequations}
subject to the condition that $p(\hat{y}_r|y_r)$ must satisfy
\begin{subequations}
\label{eq:cf_R0_constraint}
\begin{align}
R_0 \ge I(\hat{Y_r};Y_r|Y_1); \\
R_0 \ge I(\hat{Y_r};Y_r|Y_2).
\end{align}
\label{eq:cf_R0}
\end{subequations}
The key observation here is that for a general relay-interference
channel, $I(\hat{Y_r};Y_r|Y_1) \neq I(\hat{Y_r};Y_r|Y_2)$. Thus, we must set $\hat{Y_r}$ to be
such that
\begin{equation}\label{eq:cfq}
R_0 = \max \{ I(\hat{Y_r};Y_r|Y_1), I(\hat{Y_r};Y_r|Y_2) \}.
\end{equation}
Without loss of generality, assume that $I(\hat{Y_r};Y_r|Y_1)<I(\hat{Y_r};Y_r|Y_2)$.
Then for $R_2$, CF is asymptotically optimal. This is because 
$R_0 = I(\hat{Y_r};Y_r|Y_2)$, so CF and GHF are equivalent as shown in
(\ref{eq:ghf_cf}), i.e.\ both provide $R_0$ bits of rate improvement 
as $N \rightarrow 0$. However, this is not so for $R_1$. Let
\begin{equation}
R_{\Delta} = | I(\hat{Y_r};Y_r|Y_1) - I(\hat{Y_r};Y_r|Y_2)|.
\end{equation}
Then, the CF rate for $R_1$ can be computed as
\begin{eqnarray}
R_1 & = & I(X_1;Y_1,\hat{Y_r}) \NoN \\
    & = & I(X_1;Y_1) + I(\hat{Y_r};Y_r|Y_1) - I(\hat{Y_r};Y_r|X_1,Y_1) \NoN \\
    & = & I(X_1;Y_1) + R_0 - R_{\Delta} - I(\hat{Y_r};Y_r|X_1,Y_1)
\label{eq:cf_R1}
\end{eqnarray}
where the second equality follows from (\ref{eq:ghf_cf}).  Assume
again a Gaussian Wyner-Ziv quantizer $\hat{Y_r}=Y_r+\eta$ where $\eta \sim
\mathcal{N}(0,q)$. When (\ref{eq:nondeg}) is satisfied, we can 
find $q$ that satisfies (\ref{eq:cf_R0}) and is bounded away from 
zero, as can be seen from (\ref{eq:Q_2}). Thus, the $I(\hat{Y_r};Y_r|X_1,Y_1)$ 
term in (\ref{eq:cf_R1}) vanishes as $N \rightarrow 0$, as computed in
(\ref{eq:rate_loss_1}).  Therefore asymptotically, CF achieves a rate
improvement of $R_0 - R_{\Delta}$. This is not the maximal possible
rate improvement unless $R_\Delta = 0$. %$I(\hat{Y_r};Y_r|Y_1) = I(\hat{Y_r};Y_r|Y_2)$. 

We can in fact quantify the asymptotic gap by noting that the
asymptotic value of $q$ can be computed as 
\begin{equation}
q = \frac{1}{2^{2R_0}-1} \max (a, b),
\label{eq:cf_asymptotic_Q}
\end{equation}
where $a$ and $b$ are as defined in (\ref{eq:definition_ab}).
Again, assuming $I(\hat{Y_r};Y_r|Y_1) < I(\hat{Y_r};Y_r|Y_2)$, then $a < b$. 
It follows that 
\begin{equation}
R_\Delta = \frac{1}{2}  \log \left( 1 + \frac{b+a}{
	\frac{1}{2^{2R_0}-1} b +a} \right)
\end{equation}
asymptotically as $N \rightarrow 0$.

To summarize, because CF requires the auxiliary random variable to be
decodable uniquely at both receivers, the relay quantizer has to be
designed for the receiver with the worse side information. This
introduces inefficiency at the other receiver. In contrast, GHF provides 
flexibility in the choice of auxiliary random variable. It allows the 
relay quantizer to be designed for the receiver with the better side 
information. This quantizer also happens to be asymptotically optimal 
for the other receiver, thus giving us the universality of GHF.


\subsection{Rate Improvement using AF \label{app:AF}}
Finally, consider the AF relay strategy. For fair comparison, we assume
that the relay link is now an orthogonal analog broadcast channel from
the relay to the two receivers with noises $Z_1'\sim {\mathcal
N}(0,1)$ and $Z_2' \sim {\mathcal N}(0,1)$. The power constraint at
the relay $P$ is such that
\begin{equation}
  \label{eq:21}
   R_0=\frac{1}{2}\log\left(1 + P \right).
\end{equation}
In AF, the relay simply amplifies its observation $Y_r$ by a factor 
$\lambda$ and sends it through the analog broadcast channel. To
satisfy the power constraint at the relay, $\lambda$ is set as 
\begin{equation}
   \lambda = \sqrt{ \frac{P}{\Ex Y_r^2} } =
	\sqrt{ \frac{2^{2R_0}-1 }{g_1^2P_1+g_2^2P_2+N} }. 
\end{equation}
The achievable rate for the first user is then given by
\begin{align}
&R_1 = I(X_1;Y_1,\lambda Y_r+Z'_1)=\NoN \\ \NoN
&\frac{1}{2}\log\frac{\biggl\lvert
\begin{array}{cc} h_{11}^2P_1+h_{21}^2P_2+N
	&\lambda(h_{11}g_1P_1+h_{21}g_2P_2) \\
	\lambda(h_{11}g_1P_1+h_{21}g_2P_2)&
	\lambda^2(g_1^2P_1+g_2^2P_2+N)+1 \end{array}\biggr\rvert}
{\biggl\lvert\begin{array}{cc}
h_{21}^2P_2+N	&	\lambda h_{21} g_2P_2\\ 
\lambda h_{21} g_2P_2 & \lambda^2(g_2^2P_2+N)+1
\end{array}\biggr\rvert}
\end{align}
where $X_2$ is treated as noise. The rate improvement is now given by
$R_1 - I(X_1;Y_1)$.  A similar expression can be found for $R_2$. It
can be shown numerically that the rate improvement is always strictly
less than $R_0$, even as $N \rightarrow 0$. This is because AF does
not digitize the relay link, hence is always affected by the noise in
it.


\subsection{Numerical Example\label{sec:simulations}}
\begin{figure}
\centering
\includegraphics[scale=0.7]{figs/curves7}
\caption{Sum rate improvement of GHF, CF, and AF as a function of SNR
for $R_0=1$, $P=10$, $h_{11}=h_{22}=1$, $h_{12}=h_{21}=0.5$, $g_1=0.5$, 
and various values for $g_2$. The GHF and CF curves are identical for 
$g_2=0.5$. 
%solid lines represent GHF, and solid and dashed lines represent CF and
%AF, respectively. 
% GHF and CF perform similarly for a symmetric channel, but GHF outperforms CF if channel is asymmetric.
\label{fig:curves5}}
\end{figure}

Fig.~\ref{fig:curves5} shows a numerical example of the sum rate
improvements using GHF, CF, and AF, as a function of the
signal-to-noise ratio (SNR), defined as
$10\log\bigl(h_{11}^2P/N\bigr)$, for a relay-interference channel
with $R_0=1$, $P=10$, $h_{11}=h_{22}=1$, $h_{12}=h_{21}=0.5$,
$g_1=0.5$, and with various values for $g_2$. 

When the channel is symmetric, i.e., $g_2=g_1=0.5$,  GHF and CF are
identical.  Both are asymptotically optimal, i.e., the rate for each
user is asymptotically improved by $R_0$. As asymmetry is introduced, 
e.g., for $g_2=0.1$ and $g_2=0$, GHF remains asymptotically optimal,
while CF fails to be so.  

When $g_2=0.1$, we have $Y_r=0.5X_1+0.1X_2+Z_r$. Thus, $Y_r$ has 
a higher correlation with $Y_1=X_1+0.5X_2+Z_1$ as compared to
$Y_2=X_2+0.5X_1+Z_2$.
In this case, it is easier for the relay to describe its observation
to $Y_1$ than to $Y_2$ using Wyner-Ziv coding. But, a CF strategy
designed for both $Y_1$ and $Y_2$ cannot take advantage of the better
correlation at $Y_1$. It has to accommodate the user with worse side
information, as otherwise, the relay quantization codeword would not
be decodable at $Y_2$. In fact, a CF strategy designed for both $Y_1$
and $Y_2$ largely helps $Y_2$. The rate of the first user is improved 
asymptotically by about 0.2 bits, while the rate of the second user is
improved asymptotically by 1 bit. In contrast, by taking advantage of 
list decoding which does not require unique decoding of the relay
quantization codeword, GHF is able to asymptotically improve the rates 
of both users by 1 bit even when the channel is asymmetric.

An interesting scenario is the case of $g_2=0$, where the relay
observes $X_1$ only. Since the second user treats $X_1$ as noise, the
ideal relay strategy for the second user is a CF strategy that
describes the interference. The first user, however, would likely
benefit more from a decode-and-forward (DF) strategy, since the relay
observes $X_1$ with no interference. Conventional CF and DF strategies
clearly cannot be implemented simultaneously by the same relay.  The
quantize-then-hash strategy of GHF resolves this tension.
Asymptotically, it appears like a DF strategy to the first user, while
simultaneously appearing like a CF strategy to the second user.  As
Fig.~\ref{fig:curves5} shows, GHF asymptotically improves the rates of
both users by 1 bit. 

Fig.~\ref{fig:curves5} also shows the rate improvement due to AF.
Asymptotically at high SNR, AF is inferior to both CF and GHF. Note the relay quantizer introduced in Section~\ref{sec:ghf:analyze} is set to achieve asymptotic optimality, where as we could have optimized the quantizer for the entire range of noise values to achieve higher performance.  This can be done by using the alternative representation of the achievable rate in Theorem~\ref{thm:2}.



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "unirelay-master"
%%% End: 

==> unirelay-upperbounds2.tex <==
\section{Upper Bounds  \label{sec:bounds}}
% In this section we drive upper bounds on the maximum rate a common relay message could improve the sum rate. For this purpose, we use the genie aided technique developed for the interference channel in \cite{etkin_tse} and \cite{kramer_outerbounds}.

% \subsection{Weak Interference Regime:}
%In the weak interference regime, where $\INR_1<\SNR$ and $\INR_2<\SNR$, the achievable region is bounded in the following theorem:
\begin{theorem}\label{thm:boundsweak}
In the weak interference regime where $\INR_1<\SNR_1$, $\INR_2<\SNR_2$,  the capacity region of the Gaussian interference channel with an out-of-band relay  of rate $R_0$ is contained in the following region:
\begin{align}
R_1&\leq \frac{1}{2}\log\left(1+\SNR_1\right)+K_1\NoN\\
R_2&\leq \frac{1}{2}\log\left(1+\SNR_2\right)+K_2\NoN\\
R_1+R_2&\leq \frac{1}{2}\log\left(1+\SNR_1\right)+\frac{1}{2}\log\left(1+\frac{\SNR_2}{1+\INR_1}\right)+R_0+K_1\NoN\\
R_1+R_2&\leq \frac{1}{2}\log\left(1+\SNR_2\right)+\frac{1}{2}\log\left(1+\frac{\SNR_1}{1+\INR_2}\right)+R_0+K_2\NoN\\
R_1+R_2&\leq \frac{1}{2}\log\left(1+\INR_2+\frac{\SNR_1}{1+\INR_1}\right)+\frac{1}{2}\log\left(1+\INR_1+\frac{\SNR_2}{1+\INR_2}\right)+2R_0.\NoN\\
2R_1+R_2&\leq \frac{1}{2}\log\left(1+\SNR_1+\INR_2\right)+\frac{1}{2}\log\left(1+\INR_1+\frac{\SNR_2}{1+\INR_2}\right)+\frac{1}{2}\log\left(\frac{1+\SNR_1}{1+\INR_2}\right)+2R_0+K_1\NoN\\
R_1+2R_2&\leq \frac{1}{2}\log\left(1+\SNR_2+\INR_1\right)+\frac{1}{2}\log\left(1+\INR_2+\frac{\SNR_1}{1+\INR_1}\right)+\frac{1}{2}\log\left(\frac{1+\SNR_2}{1+\INR_1}\right)+2R_0+K_2,
\end{align}
where
\begin{align}
K_1&=\frac{1}{2}\log\left(\frac{1+\SNR_1+\SNR_{r1}}{1+\SNR_1}\right)\\
K_2&=\frac{1}{2}\log\left(\frac{1+\SNR_2+\SNR_{r2}}{1+\SNR_2}\right).
\end{align}
\end{theorem}
\begin{corollary}
When $\INR_{i},\SNR_{ri}<\SNR_i,i=1,2$, the capacity region is contained in the region of $(R_1,R_2)$ rate pairs defined by \eqref{eq:bounduseful}.
\end{corollary}

\begin{proof}
%First note that from the characterization of the capacity region for the Gaussian %interference channel (no relay) to within one bit in \cite[Chapter IV]{etkin_tse},
The corollary follows from the main theorem, since when $\SNR_{ri}<\SNR_i$, we have $K_i<0.5$, for $i=1,2$. The main theorem can be proved in following steps:
\BEN
\item The first bound is obtained by providing $X_2$ and $Y_r$ to destination 1. From Fano's inequality, we have:
\begin{align}
nR_1&\leq I(X_1^n;Y_1^nX_r^n)+n\epsilon\NoN\\
&\leq I(X_1^n;Y_1^nY_r^n)+n\epsilon\NoN\\
&\leq I(X_1^n;Y_1^nY_r^nX_2^n)+n\epsilon\NoN\\
&=I(X_1^n;Y_1^nY_r^n\big\vert X_2^n)+n\epsilon\NoN\\
&=I(X_1^n;h_{11}X_1^n+Z_1^n,g_1X_1^n+Z_r^n)+n\epsilon\NoN\\
&\leq nI(X_{1g};h_{11}X_{1}^G+Z_1,g_1X_{1}^G+Z_r)+n\epsilon\NoN\\
&=\frac{n}{2}\log(1+\SNR_1)+nI(X_{1}^G;g_1X_{1}^G+Z_r\big\vert h_{11}X_{1}^G+Z_1)+n\epsilon\NoN\\
&=\frac{n}{2}\log(1+\SNR_1)+\frac{n}{2}\log\left(\frac{N+h_{11}^2P_1+g_1^2P_1}{h_{11}^2P_1+N}\right)+n\epsilon\NoN\\
&=\frac{n}{2}\log(1+\SNR_1)+nK_1+n\epsilon\NoN,
\end{align}
where  $X_{1}^G$ representing a Gaussian random variable with variance $P_1$.

\item The second bound can be found by symmetry from the first bound.

\item The third bound is obtained by providing $X_2$ and $Y_r$ to destination 1. Starting from Fano's inequality, we have:
\begin{align}
n(R_1+R_2)&\leq I(X_1^n;Y_1^n X_r^n)+I(X_2^n;Y_2^nX_r^n)+n\epsilon\NoN\\
&\leq I(X_1^n;Y_1^nX_r^nX_2^nY_r^n)+I(X_2^n;Y_2^n)+I(X_2^n;X_r^n|Y_2^n)+n\epsilon\NoN\\
&\leq I(X_1^n;Y_1^nY_r^nX_2^n)+I(X_2^n;Y_2^n)+nR_0+n\epsilon\NoN\\
&= I(X_1^n;Y_1^nY_r^n|X_2^n)+I(X_2^n;Y_2^n)+nR_0+n\epsilon\NoN\\
&=I(X_1^n;Y_1^n|X_2^n)+I(X_2^n;Y_2^n)+I(X_1^n;Y_r^n|X_2^n,Y_1^n)+nR_0+n\epsilon\NoN\\
&\overset{(a)}\leq \frac{n}{2}\log\left(1+\SNR_1\right)+\frac{n}{2}\log\left(1+\frac{\SNR_2}{1+\INR_1}\right)+h\bigl(g_1X_1^n+Z_r^n\big \vert h_{11}X_1^n+Z_1^n\bigr)\NoN\\
&\hspace{8cm} -h(Z_r^n) +nR_0+n\epsilon\NoN\\
&\overset{(b)}\leq \frac{n}{2}\log\left(1+\SNR_1\right)+\frac{n}{2}\log\left(1+\frac{\SNR_2}{1+\INR_1}\right)+nh\bigl(g_1X_{1g}+Z_r\big\vert h_{11}X_{1g}+Z_1\bigr)\NoN\\
&\hspace{8cm}-nh(Z_r)+nR_0+n\epsilon\NoN\\
&=\frac{n}{2}\log(1+\SNR_1)+\frac{n}{2}\log\left(1+\frac{\SNR_2}{1+\INR_1}\right)+K_1+nR_0\NoN% \\
% &\hspace{11.5cm}+n\epsilon\NoN,\\
% &=\frac{n}{2}\log\left(1+\SNR_1\right)+\frac{n}{2}\log\left(1+\frac{\SNR_2}{1+\INR_2}\right)+\frac{n}{2}\log\left(\frac{1+\SNR_1+\SNR_{r1}}{1+\SNR_1}\right)+nR_0\NoN\\
% &\hspace{11.5cm}+n\epsilon\NoN,
\end{align}
where (a) follows from the so-called Z-channel upper bound of \cite{kramer_outerbounds} and \cite[Equation (45)]{etkin_tse}, and (b) follows from \cite[Lemma 1]{veeravalli-outerbound}.

\item The fourth bound is obtained from the third bound by symmetry.

\item The fifth bound is a trivial extension of the genie-aided bound in \cite[Section 3.4]{etkin_tse} with addition of a relay. Starting from Fano's inequality, we have:
\begin{align}
n(R_1+R_2)&\leq I(X_1^n;Y_1^n X_r^n)+I(X_2^n;Y_2^nX_r^n)+n\epsilon\NoN\\
&\leq
I(X_1^n;Y_1^n)+I(X_2^n;Y_2^n)+2h(X_r^n)+n\epsilon\NoN\\
&\leq I(X_1^n;Y_1^n)+I(X_2^n;Y_2^n)+2nR_0+n\epsilon\NoN\\
&\overset{(a)}\leq
\frac{1}{2}\log\left(1+\INR_2+\frac{\SNR_1}{1+\INR_1}\right)+\frac{1}{2}\log\left(1+\INR_1+\frac{\SNR_2}{1+\INR_2}\right)+2nR_0+n\epsilon.\NoN
\end{align}
where (a) follows from \cite[Section 3.4]{etkin_tse}.

\item The sixth bound is found using the bound on $2R_1+R_2$ \cite[Theorem 3]{etkin_tse}, and providing $X_2,Y_r$ to user one. Starting from Fano's inequality, we have:
\begin{align}
n(2R_1+R_2)&\leq I(X_1^n;Y_1^n X_r^n)+I(X_2^n;Y_2^nX_r^n)+I(X_1^n;Y_1^nX_r^n)+n\epsilon\NoN\\
&\leq
I(X_1^n;Y_1^n)+I(X_2^n;Y_2^n)+2h(X_r^n)+I(X_1^n;Y_1^nY_r^n|X_2^n) +n\epsilon\NoN\\
&\leq I(X_1^n;Y_1^n)+I(X_2^n;Y_2^n)+I(X_1^n;Y_1^nY_r^n|X_2^n)+I(X_1^n;Y_r^n|X_2^nY_1^n)+2nR_0+n\epsilon\NoN\\
&\overset{(a)}
\leq \frac{1}{2}\log\left(1+\SNR_1+\INR_2\right)+\frac{1}{2}\log\left(1+\INR_1+\frac{\SNR_2}{1+\INR_2}\right)+\frac{1}{2}\log\left(\frac{1+\SNR_1}{1+\INR_1}\right)\NoN\\
&\hspace{3cm} + h\bigl(g_1X_1^n+Z_r^n\big \vert h_{11}X_1^n+Z_1^n\bigr) -h(Z_r^n) +2nR_0+n\epsilon\NoN\NoN\\
&\overset{(b)}\leq \frac{1}{2}\log\left(1+\SNR_1+\INR_2\right)+\frac{1}{2}\log\left(1+\INR_1+\frac{\SNR_2}{1+\INR_2}\right)+\frac{1}{2}\log\left(\frac{1+\SNR_1}{1+\INR_1}\right)\NoN\\
&\hspace{3cm} + nh\bigl(g_1X_{1g}+Z_r\big\vert h_{11}X_{1g}+Z_1\bigr)-nh(Z_1) +2nR_0+n\epsilon\NoN\\
&= \frac{1}{2}\log\left(1+\SNR_1+\INR_2\right)+\frac{1}{2}\log\left(1+\INR_1+\frac{\SNR_2}{1+\INR_2}\right)+\frac{1}{2}\log\left(\frac{1+\SNR_1}{1+\INR_1}\right)\NoN\\
&\hspace{8cm} + nK_1 +2nR_0+n\epsilon\NoN.
\end{align}
where (a) follows from the bound on $2R_1+R_2$ in \cite[Theorem 3]{etkin_tse}, and (b) follows from \cite[Lemma~1]{veeravalli-outerbound}.
\item The bound on $R_1+2R_2$ is obtained from the bound on $R_1+2R_2$ by switching the 1 and 2 indices.
\EEN
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "unirelay-master4"
%%% End: 
